High-dimensional mixed-frequency IV regression

This paper introduces a high-dimensional linear IV regression for the data sampled at mixed frequencies. We show that the high-dimensional slope parameter of a high-frequency covariate can be identified and accurately estimated leveraging on a low-frequency instrumental variable. The distinguishing feature of the model is that it allows handing high-dimensional datasets without imposing the approximate sparsity restrictions. We propose a Tikhonov-regularized estimator and derive the convergence rate of its mean-integrated squared error for time series data. The estimator has a closed-form expression that is easy to compute and demonstrates excellent performance in our Monte Carlo experiments. We estimate the real-time price elasticity of supply on the Australian electricity spot market. Our estimates suggest that the supply is relatively inelastic and that its elasticity is heterogeneous throughout the day.

==> fig/tab1.tex <==
\begin{table}
	\centering
	\begin{threeparttable}
		\caption{Monte Carlo experiments for Tikhonov estimator}
		\begin{tabular}{lllrrr}
			\toprule
			$n$ & $\sigma$ & $\alpha_n$ & $\text{I-BIAS}^2(\hat \beta_{\alpha_n})$ & $\text{I-VAR}(\hat \beta_{\alpha_n})$   & $\text{MISE}(\hat \beta_{\alpha_n})$ \\
			\midrule
			100 & 0.5 & $10^{-6}$ & 0.2455 & 0.2742 & 0.5197 \\\rowcolor{gray!25}
			& 	  & $10^{-7}$ & 0.0420 & 0.4080 & 0.4500 \\
			& 	  & $10^{-8}$ & 0.0324 & 0.4545 & 0.4869 \\\rowcolor{gray!25}
			& 1.0 & $10^{-6}$ & 0.3198 & 0.4174 & 0.7372 \\
			& 	  & $10^{-7}$ & 0.0848 & 0.6595 & 0.7443 \\
			& 	  & $10^{-8}$ & 0.0669 & 0.6792 & 0.7461 \\
			500 & 0.5 & $10^{-6}$ & 0.2155 & 0.0535 & 0.2690 \\\rowcolor{gray!25}
			& 	  & $10^{-7}$ & 0.0378 & 0.0828 & 0.1206 \\
			& 	  & $10^{-8}$ & 0.0331 & 0.0884 & 0.1215 \\
			& 1.0 & $10^{-6}$ & 0.2289 & 0.0865 & 0.3154 \\
			& 	  & $10^{-7}$ & 0.0425 & 0.1215 & 0.1639 \\\rowcolor{gray!25}
			& 	  & $10^{-8}$ & 0.0319 & 0.1293 & 0.1612 \\
			1000& 0.5 & $10^{-6}$ & 0.2129 & 0.0272 & 0.2401 \\
			& 	  & $10^{-7}$ & 0.0380 & 0.0408 & 0.0788 \\\rowcolor{gray!25}
			& 	  & $10^{-8}$ & 0.0335 & 0.0423 & 0.0759 \\
			& 1.0 & $10^{-6}$ & 0.2179 & 0.0432 & 0.2611 \\
			& 	  & $10^{-7}$ & 0.0377 & 0.0606 & 0.0983 \\\rowcolor{gray!25}
			& 	  & $10^{-8}$ & 0.0335 & 0.0640 & 0.0974 \\
			\bottomrule
		\end{tabular}
		\begin{tablenotes}
			\small
			\item Note: results for different sample size $n$, noise level $\sigma$, and values of regularization parameter $\alpha_n$.
		\end{tablenotes}
		\label{tab:1}
	\end{threeparttable}
\end{table}

==> fig/tab2.tex <==
\begin{table}
	\centering
	\begin{threeparttable}
	\caption{Monte Carlo experiments for sieve estimator}
	\begin{tabular}{lllrrr}
		\toprule
		$n$ & $\sigma$ & $m_n$ & $\text{I-BIAS}^2(\hat \beta_{m_n})$ & $\text{I-VAR}(\hat \beta_{m_n})$ & $\text{MISE}(\hat \beta_{m_n})$ \\
		\midrule
		100	& 0.5 & $1$ & $8.9004$ & $0.0101$ & $8.9105$\\\rowcolor{gray!25}
			& 	  & $2$ & $0.0023$ & $0.3867$ & $0.3890$\\
			& 	  & $3$ & $0.0001$ & $1.3\times 10^5$ & $1.3\times 10^5$\\
			& 1.0 & $1$	& $8.8939$ & $0.0173$ & $8.9112$\\\rowcolor{gray!25}
			& 	  & $2$ & $0.0042$ & $0.5423$ & $0.5464$\\
			& 	  & $3$ & $0.0000$ & $1.9\times 10^5$ & $1.9\times 10^5$\\
		500 & 0.5 & $1$ & $8.9009$ & $0.0019$ & $8.9029$\\\rowcolor{gray!25}
			& 	  & $2$ & $0.0011$ & $0.0750$ & $0.0760$\\
			& 	  & $3$ & $0.0011$ & $1.8\times 10^5$ & $1.8\times 10^5$\\
			& 1.0 & $1$ & $8.9020$ & $0.0034$ & $8.9054$\\\rowcolor{gray!25}
			& 	  & $2$ & $0.0011$ & $0.0772$ & $0.0783$\\
			& 	  & $3$ & $10.1760$ & $4.0\times 10^4$ & $4.0\times 10^4$\\
		1000& 0.5 & $1$ & $8.9020$ & $0.0010$ & $8.9030$\\\rowcolor{gray!25}
			& 	  & $2$ & $0.0008$ & $0.0376$ & $0.0384$\\
			& 	  & $3$ & $8.8316$ & $0.6\times 10^5$ & $0.6\times 10^5$\\
			& 1.0 & $1$ & $8.9001$ & $0.0017$ & $8.9018$\\\rowcolor{gray!25}
			& 	  & $2$ & $0.0009$ & $0.0358$ & $0.0367$\\
			& 	  & $3$ & $233.857$ & $13.2\times 10^5$& $13.2\times 10^5$\\
		\bottomrule
	\end{tabular}
	\begin{tablenotes}
		\small
		\item Note: results for different sample size $n$, noise level $\sigma$, and values of dimension parameter $m_n$.
	\end{tablenotes}
	\label{tab:2}
	\end{threeparttable}
\end{table}
